Isospectral pairs of metrics on balls, spheres, and other manifolds with different local geometries

The first isospectral pairs of metrics are constructed on balls and spheres. This long standing problem, concerning the existence of such pairs, has been solved by a new method called "Anticommutator Technique." Among the wide range of such pairs, the most striking examples are provided on (4k-1)-dimensional spheres, where k > 2. One of these metrics is homogeneous (since it is the metric on the geodesic sphere of a 2-point homogeneous space), while the other is locally inhomogeneous. These examples demonstrate the surprising fact that no information about the isometries is encoded in the spectrum of Laplacian acting on functions. In other words, "The group of isometries, even the local homogeneity property, is lost to the "Non-Audible" in the debate of "Audible versus Non-Audible Geometry"."

==> defs.tex <==
\catcode`\@=11
\hsize=125mm
\vsize=184mm
\parskip=0pt

%%FONT SIZE=11pt

\font@\titlebf=cmbx10 scaled \magstep1
\font@\elevrm=cmr10 scaled \magstephalf
\font@\elevit=cmti10 scaled \magstephalf
\font@\elevsl=cmsl10 scaled \magstephalf
\font@\elevbf=cmbx10 scaled \magstephalf
\font@\elevi=cmmi10 scaled \magstephalf
\font@\elevsy=cmsy10 scaled \magstephalf
\font@\elevex=cmex10 scaled \magstephalf
\font@\elevbm=cmmib10 scaled \magstephalf
\font@\eightci=cmmi8
\font@\sixi=cmmi6
\font@\eightcsy=cmsy8
\font@\sixsy=cmsy6
\font@\eightcrm=cmr8
\font@\sixrm=cmr6
\font@\eightcbf=cmbx8
\font@\sixbf=cmbx6
\font@\elevsc=cmcsc10 scaled \magstephalf
\font@\ninerm=cmr9

%%EXTRA SYMBOLS

\newfam\msxfam
\newfam\msyfam
%\newfam\cmmibfam
\font@\elevmsx=msam10 scaled \magstephalf
\font@\eightmsx=msam8
\font@\sixmsx=msam6
\font@\nyolmsx=msam8
\font@\elevmsy=msbm10 scaled \magstephalf
\font@\eightmsy=msbm8
\font@\sixmsy=msbm6
\font@\nyolmsy=msbm8
\def\Bbb{\ifmmode\let\next\Bbb@\else
\def\next{\errmessage{Use \string\Bbb\space only in math mode}}\fi\next}
\def\Bbb@#1{{\Bbb@@{#1}}}
\def\Bbb@@#1{\fam\msyfam#1}

\newfam\tffam
\newtoks\elevpoint@
\def\elevpoint{\normalbaselineskip13.5\p@
\spaceskip3.5\p@ plus2\p@ minus1\p@
\abovedisplayskip13.5\p@ plus3\p@ minus9\p@
\belowdisplayskip\abovedisplayskip
\abovedisplayshortskip\z@ plus3\p@
\belowdisplayshortskip7\p@ plus3\p@ minus4\p@
\textonlyfont@\rm\elevrm \textonlyfont@\it\elevit
\textonlyfont@\sl\elevsl \textonlyfont@\bf\elevbf
\textonlyfont@\tf\elevsc %\textfont\cmmibfam\elevbm
\ifsyntax@ \def\big##1{{\hbox{$\left##1\right.$}}}%
\let\Big\big \let\bigg\big \let\Bigg\big
\else
\textfont\z@\elevrm \scriptfont\z@\eightrm
\scriptscriptfont\z@\sixrm
\textfont\@ne\elevi \scriptfont\@ne\eighti
\scriptscriptfont\@ne\sixi
\textfont\tw@\elevsy \scriptfont\tw@\eightsy
\scriptscriptfont\tw@\sixsy
\textfont\thr@@\elevex \scriptfont\thr@@\eightex
\scriptscriptfont\thr@@\eightex
\textfont\itfam\elevit \scriptfont\itfam\eightit
\scriptscriptfont\itfam\eightit
\textfont\bffam\elevbf \scriptfont\bffam\eightbf
\scriptscriptfont\bffam\sixbf
\textfont\msxfam=\elevmsx \scriptfont\msxfam=\eightmsx
\scriptscriptfont\msxfam=\sixmsx
\textfont\msyfam=\elevmsy \scriptfont\msyfam=\eightmsy
\scriptscriptfont\msyfam=\sixmsy
\setbox\strutbox\hbox{\vrule height8.5\p@ depth3.5\p@ width\z@}%
\setbox\strutbox@\hbox{\lower.5\normallineskiplimit\vbox{%
\kern-\normallineskiplimit\copy\strutbox}}%
\setbox\z@\vbox{\hbox{$($}\kern\z@}\bigsize@1.2\ht\z@
\fi
\normalbaselines\rm\dotsspace@1.5mu\ex@.2326ex\jot3\ex@
\the\elevpoint@}
\elevpoint\rm

%%PAGE OUTPUT

\NoPageNumbers
\def\lefthead{} \def\righthead{}
\headline{\ifnum\pageno=1 \hfill\else\ifodd \pageno
{\phantom{\ninerm \number\pageno}\hfill \ninerm\righthead \hfill
\ninerm\number\pageno} \else {\ninerm\number\pageno \hfill
\ninerm\lefthead\hfill\phantom{\ninerm\number\pageno}}\fi\fi}
\def\headLine#1#2{\def\lefthead{#1}\def\righthead{#2}}
\catcode`\@=12

%%DEFINITIONS

\def\bA{\bold A}
\def\bC{\bold C}
\def\bH{\bold H}
\def\bI{\bold I}
\def\bJ{\bold J}
\def\bM{\bold M}
\def\bR{\bold R}
\def\bT{\bold T}
\def\ba{\bold a}
\def\bd{\bold d}
\def\be{\bold e}
\def\bi{\bold i}
\def\bj{\bold j}
\def\bk{\bold k}
\def\bn{\bold n}
\def\bu{\bold u}
\def\bv{\bold v}
\def\bz{\bold z}
\def\b1{\bold 1}
%\def\bmu{{\boldsymbol\mu}}
\def\bmu{\hbox{\elevbm\char'26}}
\def\BH{\Bbb H}
\def\BR{\Bbb R}
\def\cF{\Cal F}
\def\cH{\Cal H}
\def\al{\alpha}
\def\ga{\gamma}
\def\de{\delta}
\def\si{\sigma}
\def\om{\omega}
\def\Ga{\Gamma}
\def\De{\Delta}
\def\ab{{(a,b)}}
\def\vab{{(a',b')}}
\def\na{\nabla}
\def\End{\operatorname{End}}
\def\SkewEnd{\operatorname{SkewEnd}}
\def\grad{\operatorname{grad}}
\def\Tr{\operatorname{Tr}}
\def\<{\langle}
\def\>{\rangle}
\def\pa{\partial}
\def\Zal{{Z^{(\al)}}}
\def\wt{\widetilde}



